Pruning Before Training May Improve Generalization, Provably

It has been observed in practice that applying pruning-at-initialization methods to neural networks and training the sparsified networks can not only retain the testing performance of the original dense models, but also sometimes even slightly boost the generalization performance. Theoretical understanding for such experimental observations are yet to be developed. This work makes the first attempt to study how different pruning fractions affect the model's gradient descent dynamics and generalization. Specifically, this work considers a classification task for overparameterized two-layer neural networks, where the network is randomly pruned according to different rates at the initialization. It is shown that as long as the pruning fraction is below a certain threshold, gradient descent can drive the training loss toward zero and the network exhibits good generalization performance. More surprisingly, the generalization bound gets better as the pruning fraction gets larger. To complement this positive result, this work further shows a negative result: there exists a large pruning fraction such that while gradient descent is still able to drive the training loss toward zero (by memorizing noise), the generalization performance is no better than random guessing. This further suggests that pruning can change the feature learning process, which leads to the performance drop of the pruned neural network.

==> main_results.tex <==
\section{Main results}
\subsection{Mild Pruning}\label{section: mild_pruning}
Our first main result shows that there exists a threshold on the pruning fraction $p$ such that pruning helps the neural network's generalization. 
\begin{theorem}[Main Theorem for Mild Pruning, Informal]\label{thm: main_thm_mild_pruning_abbr}
Under Condition \ref{condition: params} \textcolor{blue}{and some other assumption in Appendix}, choose initialization variance $\sigma_0 = \widetilde{\Theta}(m^{-4} n^{-1} \mu^{-1})$ and learning rate {$\eta \leq \widetilde{O}(1/\mu^2)$}.
For $\eps > 0$, if $p \in [C_1 \frac{\log d}{m}, 1]$ for some constant $C_1$, then with probability at least $1 - d^{-1}$, there exists $T = \widetilde{O}(K \eta^{-1} \sigma_0^{2-q} \mu^{-q} + K^2 m^4 \mu^{-2} \eta^{-1} \eps^{-1})$ such that 
\begin{enumerate}
    \item The training loss is below $\eps$: $L_S(\widetilde{\mathbf{W}}^{(T)}) \leq \eps$.
    \item The testing loss can be bounded by $ L_\mathcal{D}(\widetilde{\mathbf{W}}^{(T)}) \leq O(K \eps) + \exp(-n^2 / p)$.
\end{enumerate}
% \begin{enumerate}
%     \item The training loss is below $\eps$: $L_S(\widetilde{\mathbf{W}}^{(T)}) \leq \eps$.
%     % \item The weights of the CNN highly correlates with its corresponding class signal: $\max_{r} \gamma_{j,r, j}^{(T)} \geq \Omega(m^{-1/q})$ for all $j \in [K]$. 
%     % \item The weights of the CNN doesn't have high correlation with the signal from different classes: $\max_{j \neq k, r \in [m]} |\gamma_{j,r,k}^{(T)}| \leq \widetilde{O}(\sigma_0 \mu)$.
%     % \item None of the weights is highly correlated with the noise: $\max_{j,r,i} \zeta_{j,r,i}^{(T)} = \widetilde{O}(\sigma_0 \sigma_n \sqrt{pd}),\ \max_{j,r,i} |\omega_{j,r,i}^{(T)}| = \widetilde{O}(\sigma_0 \sigma_n \sqrt{pd})$. 
% \end{enumerate}

% \yl{Define the test loss}
\end{theorem}
\begin{remark}
The theorem indicates that there exists a threshold in the order of $\Theta(\frac{\log d}{m})$ such that if $p$ is above this threshold (i.e., the fraction of the pruned weights is small), gradient descent is able to drive the training loss towards zero and the overparameterized network achieves good testing performance. In the next subsection, we explain why pruning can help generalization via an outline of our proof, and we defer all the detailed proofs to the appendix. 
\end{remark}

\subsection{Over Pruning}
Our second result shows that there exists a relatively large pruning fraction (i.e., small $p$) such that while gradient descent is still able to drive the training error toward zero, the learned model yields poor generalization.
\begin{theorem}[Main Theorem for Over Pruning, Informal]\label{thm: main_thm_over_pruning_informal}
Under Condition \ref{condition: params} \textcolor{blue}{and some other assumption in Appendix}, choose initialization variance $\sigma_0 = \widetilde{\Theta}(m^{-4} n^{-1} \mu^{-1})$ and learning rate {$\eta \leq \widetilde{O}(1/\mu^2)$}.
For $\eps > 0$, if $p = \Theta(\frac{1}{Km \log d})$, then with probability at least $1 - 1/\poly \log d$, there exists $T = O(\eta^{-1} n \sigma_0^{q-2} \sigma_n^{-q} (pd)^{-q/2} + \eta^{-1} \eps^{-1} m^4 n \sigma_n^{-2} (pd)^{-1})$ such that 
\begin{enumerate}[itemsep=2pt,topsep=0pt,parsep=0pt]
    \item The training loss is below $\eps$: $L_S(\widetilde{\mathbf{W}}^{(T)}) \leq \eps$. 
    \item Moreover, the testing loss is large: 
    $L_\mathcal{D}(\widetilde{\mathbf{W}}^{(T)}) \geq \Omega(\log K)$.
    % \item The model weight doesn't learn any of its corresponding signal at all: $\gamma_{j,r,j}^{(t)} = 0$ for all $j \in [K],\ r \in [m]$. 
    % \item The model weights is highly correlated with the noise: $\max_{r \in [m]} \zeta_{j,r,i}^{(T)} \geq \Omega(m^{-1/q})$ if $y_i = j$. 
\end{enumerate}
\end{theorem}
\begin{remark}
The above theorem indicates that in the over-pruning case, the training loss can still go to zero. However, the testing loss of our neural network behaves no much better than random guessing, because given any sample, random guessing will assign each class with probability $1/K$, which yields a generalization loss of $\log K$.
%The second point means our neural network behaves no much better than random guessing. 
The readers might wonder why the condition for this to happen is $p = \Theta(\frac{1}{Km \log d})$ instead of $O(\frac{1}{Km \log d})$. 
Indeed, the generalization will still be bad if $p$ is too small.
However, now the neural network is not only unable to learn the signal but also can't efficiently memorize the noise via gradient descent. 
\end{remark}

==> proof.tex <==
\section{Proof Main Idea}
In this section we give an outline our proof, and we defer all the detailed proofs to the appendix. 

\subsection{Overview of the Neural Network Training in the Feature Learning Regime}
Recent development in deep learning theory has significantly advanced people's understanding on neural network training in the feature learning regime. 
Some pioneer work including \cite{allen2020towards, allen2020backward, cao2022benign, zou2021understanding,shi2021theoretical} has studied the gradient descent dynamics under the assumption that the class signal model is inherently low rank. 
Their work reveals that for classification task with cross-entropy loss, how the weight of each neuron evolves heavily depends on its property at the initialization:
If a neuron weight is heavily correlated with its corresponding class signal due to the randomness in the initialization, then its correlation will quickly grow and become one of the few large singleton neurons that detect the signal. 
The training can be roughly divided into two phases: feature learning phase and converging phase. 
In the first phase, all the weights are not far away from random initialization and thus the network's performance is bad, which means the cross-entropy loss will have large gradient.
During this phase, some of the neuron weights will change dramatically and quickly get aligned with the class signal. 
At the end of this phase, the gradient of the cross-entropy loss will become small. 
During the second phase, the neuron weights keep getting more aligned with the class signal while driving the training error and loss toward zero. 
{We point out that we use polynomial ReLU activation to help us simplify the analysis of gradient descent dynamics since polynomial ReLU activation gives a much larger separation of signal and noise than ReLU. 
We believe our analysis can be generalized to ReLU activation in the future. 
We experimentally show that our result also holds for ReLU activation. }

\subsection{Why mild pruning can improve generalization?}\label{subsection: mild_pruning}
First of all, readers might wonder why pruning can improve generalization at all. 
We first analyze the effect of pruning at the initialization.
Two very common but somehow misleading intuitions are given by the following:
\begin{itemize}
    \item Consider a fixed neuron weight. 
    If we look from an averaging (or in-expectation) perspective, at the random initialization, the signal correlation with the weights is given by $\E_{\mathbf{w,m}}[\inprod{\mathbf{w \odot m}, \boldsymbol{\mu}}] = p \sigma_0 \mu$ and the noise correlation with the weights is given by $\E_{\mathbf{w}, \mathbf{m}, \boldsymbol{\xi}}[\inprod{\mathbf{w \odot m}, \boldsymbol{\xi}}] = \sigma_0 \sigma_n \sqrt{pd}$.
    Based on this argument, pruning will hurt signal more than noise. 

    \item Since we are pruning with $\textnormal{Bernoulli}(p)$, a given neuron will not receive signal at all with probability $1 - p$ (recall that our signal model is sparse). 
    Thus, there is roughly $p$ fraction of the neurons receiving the signal and the rest $1 - p$ fraction will be purely learning from noise. 
    Even though for every neuron, roughly $\sqrt{p}$ portion of $\ell_2$ mass from the noise is reduced, at the same time, pruning also creates $1 - p$ fraction of neurons which don't receive signals at all and will purely output noise after training. 
    Summing up the contributions from every neuron, the signal strength is reduced by a factor of $p$ while the noise strength is reduced by a factor of $\sqrt{p}$.
    We again reach the conclusion of pruning under any rate will hurt the signal more than noise. 
\end{itemize}
The above analysis shows that under any pruning rate, it seems pruning can only hurt the signal more than noise at the initialization. 
The analysis will be indicative of the network after training if the network is under the neural tangent kernel regime, where the network weight doesn't travel far from its initialization and therefore the above analysis can still be hold true approximately after training. 
However, when the neural network training is in the feature learning regime, this average type analysis only capture part of the story. 
In this regime, the weight which has a large correlation with the signal at the initialization will quickly evolve into singleton neurons and those weight with small correlation will remain small. 

We also point out that our assumption on the sparsity of the signal is necessary. 
If we don't have this sparsity assumption and only make assumption on the $\ell_2$ norm of the signal, then in the extreme case, the signal is uniformly distributed across all coordinate.
In this case, the effect of pruning to the signal and the noise will be essentially the same: they will both be reduced by a factor of $\sqrt{p}$. 

Our first lemma leverages the sparsity property of our signal and shows that if the pruning is mild, then it will not hurt the max weight-signal correlation much at the initialization. 

\begin{lemma}\label{lemma: initialization_max_signal}
Suppose $p m \geq \Omega(\log (K/\delta))$, with probability $1 - \delta$, for all $j \in [K]$,
\begin{align*}
    \sigma_0 \norm{\boldsymbol{\mu}_j}_2 \leq \max_{r \in \mathcal{S}^j_\textnormal{signal}}  \inprod{\widetilde{\mathbf{w}}^{(0)}_{j,r}, \boldsymbol{\mu}_j} \leq \sqrt{2 \log (8 p m K/ \delta)} \sigma_0 \norm{\boldsymbol{\mu}_j}_2
\end{align*}
\end{lemma}
On the other hand, the max weight-noise correlation is reduced by a factor of $\sqrt{p}$. 
\begin{lemma}
With probability at least $1 - \delta$, for all $i \in [n]$, 
\begin{align*}
    \sigma_0 \sigma_n \sqrt{pd} \leq \max_r \inprod{\widetilde{\mathbf{w}}_{j,r}^{(0)}, \boldsymbol{\xi}_i} \leq \sqrt{2\log (Km/\delta)} \sigma_0 \sigma_n \sqrt{pd}
\end{align*}
\end{lemma}
Given these properties from the initialization, we leverage the existing development and prove that there exists at least one neuron that is heavily aligned with the signal after the training.  

\begin{theorem}
Under the same assumptions as Theorem \ref{thm: main_thm_mild_pruning}, within $\widetilde{O}(K \eta^{-1} \sigma_0^{2-q} \mu^{-q} + K^2 m^4 \mu^{-2} \eta^{-1} \eps^{-1})$ iterations, we can find $\widetilde{\mathbf{W}}^\star$ such that $L_S(\widetilde{\mathbf{W}}^\star) \leq \eps$ and $L_{\mathcal{D}} \leq O(K\eps) + \exp(-n^2/p)$.
\end{theorem}


\subsection{Over pruning leads to bad generalization}


==> result.tex <==
\section{Main Result}
Our first main result shows that when the pruning fraction is small (i.e., $p$ is large), pruning helps the neural network's generalization. 
\begin{theorem}[Main Theorem for Mild Pruning, Abbreviated]\label{thm: main_thm_mild_pruning}
Under Assumption \ref{assumption: params}, for $\eps > 0$, if $p \geq C \frac{\log d}{m}$ for some sufficiently large constant $C$, then with probability at least $1 - d^{-1}$, there exists $T = \widetilde{O}(K \eta^{-1} \sigma_0^{2-q} \mu^{-q} + K^2 m^4 \mu^{-2} \eta^{-1} \eps^{-1})$ such that 
\begin{enumerate}
    \item The training loss is below $\eps$: $L_S(\widetilde{\mathbf{W}}^{(T)}) \leq \eps$.
    \item Moreover, the testing loss is can be upper-bounded by 
\begin{align*}
    L_\mathcal{D}(\widetilde{\mathbf{W}}^{(T)}) \leq O(K \eps) + \exp(-n^2 / p)
\end{align*}
\end{enumerate}
% \begin{enumerate}
%     \item The training loss is below $\eps$: $L_S(\widetilde{\mathbf{W}}^{(T)}) \leq \eps$.
%     % \item The weights of the CNN highly correlates with its corresponding class signal: $\max_{r} \gamma_{j,r, j}^{(T)} \geq \Omega(m^{-1/q})$ for all $j \in [K]$. 
%     % \item The weights of the CNN doesn't have high correlation with the signal from different classes: $\max_{j \neq k, r \in [m]} |\gamma_{j,r,k}^{(T)}| \leq \widetilde{O}(\sigma_0 \mu)$.
%     % \item None of the weights is highly correlated with the noise: $\max_{j,r,i} \zeta_{j,r,i}^{(T)} = \widetilde{O}(\sigma_0 \sigma_n \sqrt{pd}),\ \max_{j,r,i} |\omega_{j,r,i}^{(T)}| = \widetilde{O}(\sigma_0 \sigma_n \sqrt{pd})$. 
% \end{enumerate}

% \yl{Define the test loss}
\end{theorem}
The improvement from pruning is showing up on the denominator of term inside the exponential. 
If $p \geq C \frac{\log d}{m}$, as $p$ gets smaller (pruning more), the generalization bound gets better. 
\textcolor{red}{May be add tightness discussion and add max signal alignment.}

Our second result shows that there exists a relatively large pruning fraction (i.e., small $p$) such that while gradient descent is still able to drive the training error toward zero, the learned model gets bad generalization.
\begin{theorem}[Main Theorem for Over Pruning, Abbreviated]\label{thm: main_thm_over_pruning}
Under Assumption \ref{assumption: params}, for $\eps > 0$, if $p = \Theta(\frac{1}{Km \log d})$, then with probability at least $1 - 1/\poly \log d$, there exists $T = O(\eta^{-1} n \sigma_0^{q-2} \sigma_n^{-q} (pd)^{-q/2} + \eta^{-1} \eps^{-1} m^4 n \sigma_n^{-2} (pd)^{-1})$ such that 
\begin{enumerate}
    \item The training loss is below $\eps$: $L_S(\widetilde{\mathbf{W}}^{(T)}) \leq \eps$. 
    \item Moreover, the testing loss is large: 
\begin{align*}
    L_\mathcal{D}(\widetilde{\mathbf{W}}^{(T)}) \geq \Omega(\log K)
\end{align*}

    % \item The model weight doesn't learn any of its corresponding signal at all: $\gamma_{j,r,j}^{(t)} = 0$ for all $j \in [K],\ r \in [m]$. 
    % \item The model weights is highly correlated with the noise: $\max_{r \in [m]} \zeta_{j,r,i}^{(T)} \geq \Omega(m^{-1/q})$ if $y_i = j$. 
\end{enumerate}
\end{theorem}
Note that given any sample, random guessing will assign each class with probability $1/K$, which leads to a generalization loss of $\log K$.
This means in this case, our neural network behaves no much better than random guessing. 
The readers might wonder why we make $p = \Theta(\frac{1}{Km \log d})$ instead of $O(\frac{1}{Km \log d})$. 
Indeed, the generalization will still be bad if we make $p$ too small but in that case the neural network is not only unable to learn the signal but also doesn't have enough capacity to memorize the noise and the objective can't be efficiently driven down toward zero. 
\begin{remark}
Judging from our results, there is a $O(K\log^2 d)$ multiplicative gap on $p$ between our two main theorems. 
We note that the gap can be narrowed down to $O(K (\log \log d)^2)$ if we want our result to hold with constant probability.
\end{remark}
